High-Resolution Chemical Abundances of the Nyx Stream

Nyx is a nearby, prograde, and high-eccentricity stellar stream physically contained in the thick disk but with an unknown origin. Nyx could be the remnant of a disrupted dwarf galaxy, in which case the associated dark matter substructure could affect terrestrial dark matter direct detection experiments. Alternatively, Nyx could be a signature of the Milky Way's disk formation and evolution. To determine the origin of Nyx, we obtained high-resolution spectroscopy of 34 Nyx stars using Keck/HIRES and Magellan/MIKE. A differential chemical abundance analysis shows that most Nyx stars reside in a metal-rich ($\mbox{[Fe/H]} > -1$) high-$\alpha$ component that is chemically indistinguishable from the thick disk. This rules out an originally suggested scenario that Nyx is the remnant of a single massive dwarf galaxy merger. However, we also identify five substantially more metal-poor stars ($\mbox{[Fe/H]} \sim -2.0$) that have chemical abundances similar to the metal-weak thick disk. It remains unclear how stars chemically identical to the thick disk can be on such prograde, high-eccentricity orbits. We suggest two most likely scenarios: that Nyx is the result of an early minor dwarf galaxy merger or that it is a record of the early spin-up of the Milky Way disk -- although neither perfectly reproduces the chemodynamic observations. The most likely formation scenarios suggest that future spectroscopic surveys should find Nyx-like structures outside of the Solar Neighborhood.

==> Table1.tex <==
\begin{longrotatetable}
\begin{deluxetable*}{lccccccccccc}
\tablecolumns{12}
\tablecaption{\label{tab:obs}Observations}
\tablewidth{800pt}
\tabletypesize{\footnotesize}
\renewcommand{\arraystretch}{1.0}
\tablehead{
\colhead{Name} & \colhead{Source id} & 
\colhead{RA} & \colhead{Dec} & 
\colhead{Obs Date} & \colhead{Instrument} & 
\colhead{$G$} & \colhead{$t_{\rm{exp}}$} & 
\colhead{SNR} & \colhead{$v_{\rm{hel}}$} &
\colhead{Score} & \colhead{Velocity}
\\ 
\colhead{} & \colhead{(\Gaia~DR3)} & 
\colhead{(degrees)} & \colhead{(degrees)} & 
\colhead{} & \colhead{} & 
\colhead{(mag)} & \colhead{(seconds)} &
\colhead{6500\AA} & \colhead{($\kms$)} &
\colhead{}& \colhead{Probability}
}
\startdata
NYX004259 & 367439335551722240  & 10.74511785  & 37.38043004  & 2020-08-01 & HIRES      & 10.74 & 350              & 151 & 24.6   & 0.97   & 0.77         \\
NYX010249 & 314182978031619328  & 15.70439781  & 32.12158685  & 2020-08-01 & HIRES      & 11.69 & 900              & 151 & 26.2   & 0.98   & 0.76         \\
NYX010842 & 306730075901451520  & 17.17457698  & 26.70320141  & 2020-08-01 & HIRES      & 11.70 & 900              & 159 & 27.1   & 0.96   & 0.78         \\
NYX013214 & 4916946665759118720 & 23.06001744  & $-51.90289781$ & 2021-01-03 & MIKE       & 10.18 & 1200             & 140 & $-16.2$  & 0.97   & 0.97         \\
NYX014107 & 317636063018105088  & 25.27974372  & 33.92092371  & 2020-08-01 & HIRES      & 11.21 & 550              & 144 & 27.1   & 0.97   & 0.61         \\
NYX014725 & 305238279140992896  & 26.85528438  & 32.42734287  & 2020-08-01 & HIRES      & 8.88  & 70               & 145 & 27.4   & 0.96   & 0.89         \\
NYX022545 & 5174773415097847296 & 36.43952571  & $-10.98901054$ & 2020-08-01 & HIRES      & 11.62 & 900              & 148 & 26.3   & 0.96   & 0.94         \\
NYX035539 & 4665853149532721664 & 58.91244399  & $-71.36549004$ & 2021-01-03 & MIKE       & 11.04 & 4085             & 232 & $-4.0$     & 0.95   & 0.95         \\
NYX044831 & 4665093769251640704 & 72.13076827  & $-62.48367570$ & 2021-01-03 & MIKE       & 8.91  & 400              & 169 & $-4.4$   & 0.98   & 0.96         \\
NYX063721 & 5497838651784528000 & 99.33851551  & $-54.82999871$ & 2021-01-04 & MIKE       & 10.52 & 1600             & 213 & 1.4    & 0.97   & 0.80         \\
NYX064943 & 5497618547596953472 & 102.43003976 & $-53.84094205$ & 2021-01-03 & MIKE       & 9.03  & 600              & 248 & 2.5    & 0.98   & 0.97         \\
NYX122147 & 3521755401833022080 & 185.44804146 & $-15.12392540$ & 2021-07-28 & MIKE       & 11.48 & 1800             & 121 & 2.8    & 0.97   & 0.97         \\
NYX163705 & 1312596465842920576 & 249.27099451 & 31.32412562  & 2020-08-01 & HIRES      & 11.93 & 1000             & 144 & $-16.7$  & 1.00   & 0.82         \\
NYX175752 & 4609530533258729600 & 269.46600702 & 36.54835952  & 2020-08-01 & HIRES      & 10.65 & 300              & 155 & $-9.6$   & 0.97   & 0.95         \\
NYX175906 & 1345377378530252032 & 269.77384034 & 42.85162989  & 2020-08-01 & HIRES      & 12.33 & 1500             & 137 & $-7.6$   & 0.98   & 0.97         \\
NYX185206 & 2146631118469602944 & 283.02543696 & 53.80289724  & 2020-08-01 & HIRES      & 9.67  & 180              & 190 & $-0.9$   & 0.98   & 0.95         \\
NYX185250 & 2103594068696931968 & 283.21008746 & 40.77249320  & 2020-08-01 & HIRES      & 12.54 & 1800             & 149 & $-3.9$   & 0.97   & 0.87         \\
NYX195253 & 4195105698600078848 & 298.22200157 & $-9.45925775$  & 2020-08-01 & HIRES      & 12.46 & 1800             & 148 & $-5.6$   & 0.97   & 0.93         \\
NYX201634 & 2062121830140100992 & 304.14213600 & 39.18034350  & 2020-08-01 & HIRES      & 11.27 & 600              & 159 & 3.4    & 0.98   & 0.88         \\
NYX201856 & 2084248913225887104 & 304.73284567 & 48.34020559  & 2020-08-01 & HIRES      & 11.91 & 1000             & 143 & 4.7    & 0.97   & 0.97         \\
NYX204828 & 1751338782564204672 & 312.11838846 & 9.68257413   & 2020-08-01 & HIRES      & 10.14 & 300              & 179 & 3.6    & 0.97   & 0.88         \\
NYX205642 & 1757797833557540480 & 314.17519078 & 12.37187691  & 2020-08-01 & HIRES      & 12.04 & 1200             & 155 & 5.0      & 0.96   & 0.94         \\
NYX211145 & 1867283181371868544 & 317.93598233 & 35.27867523  & 2020-08-01 & HIRES      & 11.71 & 900              & 162 & 8.6    & 0.98   & 0.94         \\
NYX213012 & 1850722646463457920 & 322.55098693 & 31.10214042  & 2020-08-01 & HIRES      & 12.44 & 1800             & 148 & 10.3   & 0.99   & 0.93         \\
NYX214142 & 1797966051335964672 & 325.42542891 & 25.19027732  & 2020-08-01 & HIRES      & 11.39 & 600              & 142 & 11.2   & 0.98   & 0.97         \\
NYX215612 & 2695833495753971072 & 329.04880607 & 3.77654551   & 2020-08-01 & HIRES      & 12.81 & 2160             & 134 & 11.2   & 0.96   & 0.91         \\
NYX215744 & 1794930334091349632 & 329.43432692 & 23.58644105  & 2020-08-01 & HIRES      & 10.72 & 350              & 150 & 12.8   & 1.00   & 0.96         \\
NYX223035 & 2738050790890416384 & 337.64587000 & 18.37272779  & 2020-08-01 & HIRES      & 11.33 & 600              & 147 & 16     & 0.96   & 0.91         \\
NYX224245 & 2833632062543310848 & 340.68697508 & 19.16973836  & 2020-08-01 & HIRES      & 10.83 & 400              & 142 & 17.2   & 0.98   & 0.95         \\
NYX225510 & 2714860681911345280 & 343.79139075 & 9.53497180   & 2020-08-01 & HIRES      & 11.16 & 1200             & 215 & 17.9   & 0.95   & 0.90         \\
NYX230605 & 2815219469025808128 & 346.52177833 & 13.86879634  & 2020-08-01 & HIRES      & 11.20 & 500              & 140 & 19.3   & 0.97   & 0.91         \\
NYX230903 & 2385788396590080512 & 347.26428804 & $-23.09773201$ & 2020-08-01 & HIRES      & 11.67 & 900              & 150 & 14.1   & 0.97   & 0.87         \\
NYX232032 & 2813625898720075264 & 350.13478016 & 13.36493995  & 2020-08-01 & HIRES      & 9.05  & 80               & 153 & 20.5   & 0.96   & 0.93         \\
NYX234631 & 2771034730974538624 & 356.62832066 & 14.41544640  & 2020-08-01 & HIRES      & 12.58 & 1800             & 141 & 22.7   & 0.97   & 0.91
\enddata
\end{deluxetable*}
\end{longrotatetable}

==> Table2.tex <==
\begin{deluxetable*}{lccccccccccccccc}
\tablecolumns{15}
\tabletypesize{\footnotesize}
\tablecaption{\label{tab:lines}Line Measurements}
\tablehead{Star & $\lambda$ (\AA) & ID & $\chi$ & $\log gf$ & EW & $\sigma$(EW) & FWHM (\AA) & $\log \epsilon_{i\,,\mathrm{ref}}$ & $d_i$ & $e_i$ 
& $\delta_{i,\teff}$ & $\delta_{i,\logg}$ & $\delta_{i,\nu_t}$ & $\delta_{i,\text{[M/H]}}$ 
}
\startdata
NYX201856   & 5778.45 &  26.0 &   2.59  & $ -3.43 $ &   9.5 &  0.4 &  0.11 & $ 6.92$ & $-0.35$ &  0.02 & $+0.05$ & $-0.00$ & $-0.00$ & $+0.01$ \\
NYX201856   & 5855.08 &  26.0 &   4.61  & $ -1.48 $ &   8.7 &  0.4 &  0.15 & $ 6.96$ & $-0.29$ &  0.02 & $+0.03$ & $+0.00$ & $-0.00$ & $+0.01$ \\
NYX201856   & 6027.05 &  26.0 &   4.08  & $ -1.09 $ &  40.5 &  0.3 &  0.13 & $ 7.00$ & $-0.31$ &  0.01 & $+0.04$ & $+0.00$ & $-0.02$ & $+0.02$ \\
NYX201856   & 6136.99 &  26.0 &   2.20  & $ -2.95 $ &  47.2 &  0.3 &  0.13 & $ 7.02$ & $-0.30$ &  0.01 & $+0.06$ & $+0.00$ & $-0.03$ & $+0.01$ \\
NYX201856   & 6151.62 &  26.0 &   2.18  & $ -3.29 $ &  30.3 &  0.3 &  0.12 & $ 6.97$ & $-0.31$ &  0.01 & $+0.06$ & $+0.00$ & $-0.01$ & $+0.01$ \\
NYX201856   & 6165.36 &  26.0 &   4.14  & $ -1.47 $ &  21.1 &  0.3 &  0.12 & $ 6.97$ & $-0.31$ &  0.01 & $+0.03$ & $+0.00$ & $-0.01$ & $+0.01$ \\
NYX201856   & 6173.33 &  26.0 &   2.22  & $ -2.88 $ &  47.4 &  0.4 &  0.12 & $ 6.98$ & $-0.30$ &  0.01 & $+0.06$ & $+0.00$ & $-0.03$ & $+0.01$ \\
NYX201856   & 6213.43 &  26.0 &   2.22  & $ -2.48 $ &  62.8 &  0.4 &  0.14 & $ 6.92$ & $-0.28$ &  0.01 & $+0.07$ & $+0.00$ & $-0.04$ & $+0.01$ \\
NYX201856   & 6271.28 &  26.0 &   3.33  & $ -2.70 $ &  11.7 &  0.4 &  0.15 & $ 6.94$ & $-0.24$ &  0.02 & $+0.04$ & $-0.00$ & $-0.00$ & $+0.01$ \\
NYX201856   & 6322.69 &  26.0 &   2.59  & $ -2.43 $ &  52.6 &  0.4 &  0.14 & $ 7.03$ & $-0.30$ &  0.01 & $+0.06$ & $+0.00$ & $-0.03$ & $+0.02$ \\
NYX201856   & 6335.33 &  26.0 &   2.20  & $ -2.18 $ &  76.8 &  0.4 &  0.15 & $ 6.87$ & $-0.25$ &  0.01 & $+0.08$ & $-0.00$ & $-0.05$ & $+0.01$ \\
NYX201856   & 6411.65 &  26.0 &   3.65  & $ -0.60 $ &  89.2 &  0.5 &  0.17 & $ 6.89$ & $-0.26$ &  0.01 & $+0.06$ & $-0.03$ & $-0.03$ & $+0.04$ \\
NYX201856   & 6518.37 &  26.0 &   2.83  & $ -2.44 $ &  37.7 &  0.4 &  0.14 & \nodata & \nodata &  0.01 & $+0.05$ & $+0.00$ & $-0.02$ & $+0.01$ \\
NYX201856   & 6581.21 &  26.0 &   1.49  & $ -4.68 $ &   9.2 &  0.4 &  0.13 & $ 7.01$ & $-0.42$ &  0.02 & $+0.06$ & $-0.00$ & $-0.00$ & $+0.01$ \\
NYX201856   & 6593.87 &  26.0 &   2.43  & $ -2.42 $ &  62.2 &  0.4 &  0.15 & $ 7.02$ & $-0.26$ &  0.01 & $+0.07$ & $+0.00$ & $-0.04$ & $+0.01$ \\
NYX201856   & 6609.11 &  26.0 &   2.56  & $ -2.69 $ &  41.4 &  0.4 &  0.14 & $ 7.01$ & $-0.32$ &  0.01 & $+0.06$ & $+0.00$ & $-0.02$ & $+0.01$ \\
NYX201856   & 6739.52 &  26.0 &   1.56  & $ -4.79 $ &   7.5 &  0.4 &  0.18 & $ 6.89$ & $-0.21$ &  0.03 & $+0.06$ & $-0.00$ & $-0.00$ & $+0.01$ \\
NYX201856   & 6810.26 &  26.0 &   4.61  & $ -0.99 $ &  22.1 &  0.4 &  0.15 & $ 6.98$ & $-0.34$ &  0.01 & $+0.03$ & $+0.00$ & $-0.01$ & $+0.02$ \\
NYX201856   & 6828.59 &  26.0 &   4.64  & $ -0.82 $ &  27.6 &  0.4 &  0.16 & $ 6.98$ & $-0.32$ &  0.01 & $+0.03$ & $+0.00$ & $-0.01$ & $+0.02$ \\
NYX201856   & 6837.01 &  26.0 &   4.59  & $ -1.69 $ &   7.2 &  0.4 &  0.18 & $ 7.01$ & $-0.26$ &  0.03 & $+0.03$ & $+0.00$ & $-0.00$ & $+0.01$ \\
NYX201856   & 6843.66 &  26.0 &   4.55  & $ -0.73 $ &  31.7 &  0.3 &  0.14 & $ 6.88$ & $-0.32$ &  0.01 & $+0.03$ & $+0.00$ & $-0.01$ & $+0.02$ \\
\enddata
\tablecomments{A portion of this table is shown for form. Column details are provided in the text. The full version is available online.}
\end{deluxetable*}


==> Table3.tex <==
\begin{deluxetable*}{lcccccccccc}
\tablecolumns{11}
\tabletypesize{\footnotesize}
\tablecaption{\label{tab:sp}Stellar Parameters}
\tablehead{ Star & $\teff (\unit{K})$ & $\sigma(\teff)$ & $\log g$ (dex) & $\sigma(\log g)$ & $\nu_t (\kms)$ & $\sigma(\nu_t)$ & $\mbox{[M/H]}$ & $\sigma(\mbox{[M/H]})$ & $\mbox{\alphafe}$ & $\text{[Fe/H]}\textsubscript{d}$ }
\startdata
NYX004259   & 6400 &  177 &  4.10 &  0.16 &  1.60 &  0.23 & $-0.45$ &  0.11 &  0.30 & $-0.30$ \\
NYX010249   & 6154 &  280 &  3.90 &  0.20 &  1.01 &  1.05 & $-2.26$ &  0.14 &  0.40 & $-2.20$ \\
NYX010842   & 4980 &   94 &  3.45 &  0.15 &  0.89 &  0.11 & $-0.50$ &  0.13 &  0.40 & $-0.42$ \\
NYX013214   & 5296 &   97 &  4.07 &  0.17 &  0.82 &  0.24 & $-1.01$ &  0.13 &  0.40 & $-0.86$ \\
NYX014107   & 5082 &   77 &  2.64 &  0.15 &  1.48 &  0.09 & $-0.75$ &  0.12 &  0.40 & $-0.68$ \\
NYX014725   & 5120 &   90 &  3.09 &  0.16 &  1.19 &  0.09 & $-0.31$ &  0.12 &  0.40 & $-0.22$ \\
NYX022545   & 4734 &  100 &  2.92 &  0.18 &  1.16 &  0.10 & $-0.39$ &  0.13 &  0.40 & $-0.32$ \\
NYX035539   & 4513 &   74 &  2.22 &  0.16 &  1.43 &  0.09 & $-0.74$ &  0.12 &  0.40 & $-0.67$ \\
NYX044831   & 5314 &   69 &  2.60 &  0.15 &  1.70 &  0.11 & $-0.93$ &  0.11 &  0.40 & $-0.86$ \\
NYX063721   & 4984 &   76 &  2.77 &  0.16 &  1.38 &  0.09 & $-0.56$ &  0.12 &  0.40 & $-0.47$ \\
NYX064943   & 4638 &   87 &  2.12 &  0.17 &  1.50 &  0.09 & $-0.44$ &  0.13 &  0.40 & $-0.36$ \\
NYX122147   & 4652 &   71 &  1.54 &  0.15 &  1.32 &  0.15 & $-2.19$ &  0.13 &  0.40 & $-2.13$ \\
NYX163705   & 5530 &   88 &  4.54 &  0.16 &  0.85 &  0.20 & $-0.60$ &  0.12 &  0.40 & $-0.47$ \\
NYX175752   & 4445 &   69 &  2.04 &  0.21 &  1.61 &  0.09 & $-0.57$ &  0.12 &  0.40 & $-0.49$ \\
NYX175906   & 5870 &  117 &  3.85 &  0.19 &  0.85 &  0.64 & $-1.78$ &  0.14 &  0.40 & $-1.71$ \\
NYX185250   & 5228 &   75 &  2.89 &  0.16 &  1.59 &  0.10 & $-0.74$ &  0.12 &  0.40 & $-0.66$ \\
NYX195253   & 5623 &   93 &  3.85 &  0.16 &  1.12 &  0.14 & $-0.70$ &  0.12 &  0.40 & $-0.56$ \\
NYX201634   & 4933 &   70 &  3.10 &  0.15 &  1.08 &  0.08 & $-0.75$ &  0.12 &  0.40 & $-0.67$ \\
NYX201856   & 5402 &   68 &  3.71 &  0.15 &  0.90 &  0.11 & $-0.84$ &  0.11 &  0.40 & $-0.70$ \\
NYX204828   & 4541 &   70 &  2.21 &  0.16 &  1.37 &  0.09 & $-0.80$ &  0.12 &  0.40 & $-0.71$ \\
NYX205642   & 5135 &   71 &  3.73 &  0.15 &  1.07 &  0.09 & $-0.55$ &  0.11 &  0.40 & $-0.47$ \\
NYX211145   & 4884 &   75 &  3.07 &  0.16 &  1.27 &  0.09 & $-0.66$ &  0.12 &  0.40 & $-0.58$ \\
NYX213012   & 5003 &   76 &  2.52 &  0.15 &  0.91 &  0.17 & $-2.14$ &  0.12 &  0.40 & $-2.08$ \\
NYX214142   & 5188 &   69 &  2.75 &  0.15 &  1.49 &  0.09 & $-0.83$ &  0.11 &  0.40 & $-0.74$ \\
NYX215612   & 5789 &  111 &  4.22 &  0.15 &  1.26 &  0.21 & $-0.63$ &  0.12 &  0.40 & $-0.51$ \\
NYX215744   & 4990 &   85 &  3.65 &  0.16 &  0.92 &  0.12 & $-0.28$ &  0.12 &  0.40 & $-0.20$ \\
NYX223035   & 4905 &   73 &  2.72 &  0.16 &  1.31 &  0.09 & $-0.45$ &  0.12 &  0.40 & $-0.38$ \\
NYX224245   & 4985 &  114 &  3.67 &  0.15 &  0.80 &  0.14 & $-0.21$ &  0.13 &  0.40 & $-0.13$ \\
NYX225510   & 5584 &   86 &  3.84 &  0.15 &  1.10 &  0.13 & $-0.79$ &  0.11 &  0.40 & $-0.66$ \\
NYX230605   & 6501 &  118 &  3.84 &  0.17 &  1.40 &  0.19 & $-0.56$ &  0.11 &  0.25 & $-0.42$ \\
NYX230903   & 5401 &   68 &  3.55 &  0.16 &  0.96 &  0.11 & $-1.41$ &  0.11 &  0.30 & $-1.35$ \\
NYX232032   & 5032 &   74 &  3.16 &  0.16 &  1.14 &  0.09 & $-0.88$ &  0.12 &  0.40 & $-0.80$ \\
NYX234631   & 5612 &  121 &  3.70 &  0.17 &  0.79 &  0.28 & $-0.96$ &  0.13 &  0.40 & $-0.82$ \\
Arcturus    & 4290 &  119 &  1.60 &  0.31 &  1.60 &  0.22 & $-0.50$ &  0.14 &  0.40 & $-0.49$ \\
HIP7162     & 5217 &   92 &  2.97 &  0.16 &  1.60 &  0.49 & $-2.05$ &  0.12 &  0.40 & $-2.05$ \\
HIP88622    & 5754 &   80 &  4.32 &  0.15 &  1.00 &  0.13 & $-0.53$ &  0.11 &  0.40 & $-0.40$ \\
\enddata
\tablecomments{Stellar parameters of the Nyx stars. $\text{{[X/Fe]}d}$ refers to the differential Fe abundance, which differs from the model metallicity $\text{{[M/H]}}$. \textbf{
See Sec.~\ref{sec:method} for more details.}}
\end{deluxetable*}

==> Table4.tex <==
\begin{deluxetable*}{llcccccccccc}
\tablecolumns{12}
\tabletypesize{\footnotesize}
\tablecaption{\label{tab:abunds}Stellar Abundances}
\setlength{\tabcolsep}{3pt}
\tablehead{Star & El. & $N$ & 
$\text{[X/H]}\textsubscript{d}$ &
$\text{{[X/Fe]}}\textsubscript{d}$ & $\sigma_{\text{{[X/Fe]}d}}$ &
$\text{[X/H]}\textsubscript{ref}$ &
$\sigma_{\text{{[X/H]}}}\textsubscript{ref}$ &
$\text{[X/Fe]}\textsubscript{ref}$ &
$\sigma_{\mathrm{rand}}$ &
$\sigma_{\mathrm{sys}}$ &
$\sigma_{\mathrm{sp}}$
}
\startdata
NYX201856       & Na I  &   4 & $-0.68$ & $ 0.02$ &  0.06 &$-0.37$ &  0.02 & $ 0.03$ & 0.00 &  0.04 &  0.04 \\
NYX201856       & Mg I  &   4 & $-0.34$ & $ 0.36$ &  0.06 &$-0.15$ &  0.02 & $ 0.25$ & 0.00 &  0.02 &  0.06 \\
NYX201856       & Si I  &   6 & $-0.55$ & $ 0.14$ &  0.12 &$-0.23$ &  0.03 & $ 0.17$ & 0.00 &  0.12 &  0.03 \\
NYX201856       & Ca I  &   7 & $-0.46$ & $ 0.24$ &  0.07 &$-0.29$ &  0.02 & $ 0.11$ & 0.00 &  0.02 &  0.07 \\
NYX201856       & Ti I  &  25 & $-0.37$ & $ 0.33$ &  0.09 &$-0.19$ &  0.01 & $ 0.21$ & 0.00 &  0.05 &  0.07 \\
NYX201856       & Fe I  &  20 & $-0.70$ & $ 0.00$ &  0.07 &$-0.40$ &  0.01 & $ 0.00$ & 0.00 &  0.04 &  0.06 \\
NYX201856       & Fe II &   5 & \nodata & \nodata &  0.11 &\nodata & \nodata & \nodata & 0.01 &  0.05 &  0.09 \\
NYX201856       & Ni I  &  12 & $-0.69$ & $ 0.01$ &  0.07 &$-0.40$ &  0.01 & $ 0.00$ & 0.00 &  0.04 &  0.06 \\
NYX201856       & Zn I  &   2 & $-0.53$ & $ 0.17$ &  0.08 &$-0.22$ &  0.02 & $ 0.18$ & 0.01 &  0.02 &  0.08 \\
NYX201856       & Y II  &   3 & $-0.66$ & $ 0.04$ &  0.10 &$-0.56$ &  0.03 & $-0.16$ & 0.01 &  0.05 &  0.09 \\
NYX201856       & Ba II &   3 & $-0.68$ & $ 0.02$ &  0.10 &$-0.47$ &  0.04 & $-0.07$ & 0.00 &  0.04 &  0.10 \\
\enddata
\tablecomments{One star from this table is shown for form. Column details are provided in the text. The full version is available online.
}
\end{deluxetable*}


==> Table4_Extended.tex <==
\begin{deluxetable*}{llcccccccccc}
\tablecolumns{12}
\tabletypesize{\footnotesize}
\tablecaption{\label{tab:abunds}Stellar Abundances}
\tablehead{Star & El. & $N$ & $\text{[X/H]}\textsubscript{d}$ & $\text{[X/Fe]}\textsubscript{d}$ & $\sigma_{\text{{[X/Fe]}d}}$  & $\text{[X/H]}\textsubscript{ref}$ & $\sigma_{\text{{[X/H]}}}\textsubscript{ref}$ & $\text{[X/Fe]}\textsubscript{ref}$ &$\sigma_{\mathrm{rand}}$ & $\sigma_{\mathrm{sys}}$ & $\sigma_{\mathrm{sp}}$}
\startdata
NYX004259       & Na I  &   1 & $-0.05$ & $ 0.24$ &  0.09 &$-0.37$ &  0.02 & $ 0.03$ & 0.01 &  0.00 &  0.09 \\
NYX004259       & Mg I  &   2 & $-0.10$ & $ 0.20$ &  0.14 &$-0.15$ &  0.02 & $ 0.25$ & 0.01 &  0.07 &  0.13 \\
NYX004259       & Si I  &   4 & $-0.22$ & $ 0.07$ &  0.15 &$-0.23$ &  0.03 & $ 0.17$ & 0.01 &  0.13 &  0.07 \\
NYX004259       & Ca I  &   5 & $-0.19$ & $ 0.11$ &  0.13 &$-0.29$ &  0.02 & $ 0.11$ & 0.01 &  0.03 &  0.13 \\
NYX004259       & Ti I  &  11 & $-0.11$ & $ 0.19$ &  0.16 &$-0.19$ &  0.01 & $ 0.21$ & 0.00 &  0.06 &  0.15 \\
NYX004259       & Fe I  &  10 & $-0.30$ & $ 0.00$ &  0.13 &$-0.40$ &  0.01 & $ 0.00$ & 0.01 &  0.04 &  0.12 \\
NYX004259       & Fe II &   3 & \nodata & \nodata &  0.09 &\nodata & \nodata & \nodata & 0.01 &  0.06 &  0.07 \\
NYX004259       & Ni I  &   7 & $-0.26$ & $ 0.04$ &  0.16 &$-0.40$ &  0.01 & $ 0.00$ & 0.01 &  0.11 &  0.11 \\
NYX004259       & Zn I  &   2 & $-0.28$ & $ 0.01$ &  0.10 &$-0.22$ &  0.02 & $ 0.18$ & 0.01 &  0.01 &  0.10 \\
NYX004259       & Y II  &   2 & $-0.38$ & $-0.08$ &  0.09 &$-0.56$ &  0.03 & $-0.16$ & 0.02 &  0.01 &  0.09 \\
NYX004259       & Ba II &   2 & $-0.32$ & $-0.02$ &  0.11 &$-0.47$ &  0.04 & $-0.07$ & 0.01 &  0.02 &  0.11 \\
NYX010249       & Na I  &   1 & $-2.06$ & $ 0.14$ &  0.14 &$-2.23$ &  0.08 & $-0.18$ & 0.04 &  0.00 &  0.13 \\
NYX010249       & Mg I  &   2 & $-1.70$ & $ 0.50$ &  0.30 &$-1.69$ &  0.03 & $ 0.36$ & 0.01 &  0.02 &  0.30 \\
NYX010249       & Ca I  &   5 & $-1.83$ & $ 0.37$ &  0.20 &$-1.84$ &  0.05 & $ 0.21$ & 0.01 &  0.06 &  0.19 \\
NYX010249       & Ti I  &   9 & $-1.81$ & $ 0.39$ &  0.32 &$-1.89$ &  0.10 & $ 0.16$ & 0.01 &  0.12 &  0.29 \\
NYX010249       & Fe I  &   8 & $-2.20$ & $ 0.00$ &  0.28 &$-2.05$ &  0.06 & $ 0.00$ & 0.01 &  0.14 &  0.24 \\
NYX010249       & Fe II &   6 & \nodata & \nodata &  0.16 &\nodata & \nodata & \nodata & 0.01 &  0.05 &  0.15 \\
NYX010249       & Ni I  &   3 & $-2.40$ & $-0.20$ &  0.22 &$-2.17$ &  0.08 & $-0.12$ & 0.01 &  0.01 &  0.22 \\
NYX010249       & Zn I  &   2 & \nodata & \nodata &  0.22 &\nodata & \nodata & \nodata & 0.02 &  0.12 &  0.19 \\
NYX010249       & Y II  &   1 & $-2.09$ & $ 0.11$ &  0.21 &$-2.23$ &  0.18 & $-0.18$ & 0.03 &  0.00 &  0.21 \\
NYX010249       & Ba II &   2 & $-2.53$ & $-0.33$ &  0.25 &$-2.22$ &  0.18 & $-0.17$ & 0.01 &  0.02 &  0.25 \\
NYX010842       & Na I  &   4 & $-0.47$ & $-0.05$ &  0.15 &$-0.40$ & \nodata & $ 0.09$ & 0.00 &  0.11 &  0.11 \\
NYX010842       & Mg I  &   4 & $-0.06$ & $ 0.36$ &  0.14 &$-0.10$ & \nodata & $ 0.39$ & 0.00 &  0.09 &  0.10 \\
NYX010842       & Si I  &   4 & $-0.14$ & $ 0.28$ &  0.09 &$-0.14$ & \nodata & $ 0.35$ & 0.00 &  0.03 &  0.08 \\
NYX010842       & Ca I  &   7 & $-0.21$ & $ 0.20$ &  0.16 &$-0.28$ & \nodata & $ 0.21$ & 0.00 &  0.05 &  0.15 \\
NYX010842       & Ti I  &  12 & $-0.12$ & $ 0.30$ &  0.18 &$-0.23$ & \nodata & $ 0.26$ & 0.00 &  0.07 &  0.17 \\
NYX010842       & Fe I  &  22 & $-0.42$ & $ 0.00$ &  0.13 &$-0.49$ & \nodata & $ 0.00$ & 0.00 &  0.05 &  0.12 \\
NYX010842       & Fe II &   7 & $-0.32$ & $ 0.10$ &  0.22 &$-0.40$ & \nodata & $ 0.09$ & 0.00 &  0.05 &  0.21 \\
NYX010842       & Ni I  &   6 & $-0.37$ & $ 0.05$ &  0.13 &$-0.45$ & \nodata & $ 0.04$ & 0.00 &  0.05 &  0.12 \\
NYX010842       & Zn I  &   2 & $-0.04$ & $ 0.38$ &  0.14 &$-0.29$ & \nodata & $ 0.20$ & 0.01 &  0.03 &  0.13 \\
NYX010842       & Y II  &   3 & $-0.44$ & $-0.02$ &  0.17 &$-0.71$ & \nodata & $-0.22$ & 0.01 &  0.05 &  0.16 \\
NYX010842       & Ba II &   3 & $-0.45$ & $-0.04$ &  0.17 &$-0.66$ & \nodata & $-0.17$ & 0.00 &  0.07 &  0.15 \\
NYX010842       & La II &   1 & $-0.40$ & $ 0.02$ &  0.17 &$-0.57$ & \nodata & $-0.08$ & 0.05 &  0.00 &  0.16 \\
NYX013214       & Na I  &   4 & $-0.70$ & $ 0.15$ &  0.08 &$-0.37$ &  0.02 & $ 0.03$ & 0.01 &  0.04 &  0.06 \\
NYX013214       & Mg I  &   4 & $-0.54$ & $ 0.31$ &  0.11 &$-0.15$ &  0.02 & $ 0.25$ & 0.01 &  0.07 &  0.08 \\
NYX013214       & Si I  &   6 & $-0.70$ & $ 0.16$ &  0.14 &$-0.23$ &  0.03 & $ 0.17$ & 0.01 &  0.14 &  0.04 \\
NYX013214       & Ca I  &   7 & $-0.53$ & $ 0.32$ &  0.11 &$-0.29$ &  0.02 & $ 0.11$ & 0.00 &  0.02 &  0.11 \\
NYX013214       & Ti I  &  23 & $-0.58$ & $ 0.28$ &  0.14 &$-0.19$ &  0.01 & $ 0.21$ & 0.00 &  0.08 &  0.12 \\
NYX013214       & Fe I  &  18 & $-0.86$ & $ 0.00$ &  0.11 &$-0.40$ &  0.01 & $ 0.00$ & 0.00 &  0.07 &  0.08 \\
NYX013214       & Fe II &   4 & \nodata & \nodata &  0.14 &\nodata & \nodata & \nodata & 0.01 &  0.08 &  0.11 \\
NYX013214       & Ni I  &  11 & $-0.87$ & $-0.02$ &  0.11 &$-0.40$ &  0.01 & $ 0.00$ & 0.00 &  0.07 &  0.08 \\
NYX013214       & Zn I  &   2 & $-0.66$ & $ 0.19$ &  0.08 &$-0.22$ &  0.02 & $ 0.18$ & 0.01 &  0.01 &  0.08 \\
NYX013214       & Y II  &   3 & $-0.88$ & $-0.03$ &  0.15 &$-0.56$ &  0.03 & $-0.16$ & 0.01 &  0.12 &  0.10 \\
NYX013214       & Ba II &   3 & $-0.94$ & $-0.08$ &  0.13 &$-0.47$ &  0.04 & $-0.07$ & 0.01 &  0.05 &  0.12 \\
NYX014107       & Na I  &   4 & $-0.68$ & $-0.00$ &  0.11 &$-0.40$ & \nodata & $ 0.09$ & 0.00 &  0.07 &  0.08 \\
NYX014107       & Mg I  &   3 & $-0.36$ & $ 0.32$ &  0.11 &$-0.10$ & \nodata & $ 0.39$ & 0.00 &  0.02 &  0.11 \\
NYX014107       & Si I  &   4 & $-0.33$ & $ 0.34$ &  0.06 &$-0.14$ & \nodata & $ 0.35$ & 0.00 &  0.03 &  0.06 \\
NYX014107       & Ca I  &   7 & $-0.37$ & $ 0.30$ &  0.14 &$-0.28$ & \nodata & $ 0.21$ & 0.00 &  0.07 &  0.12 \\
NYX014107       & Ti I  &  10 & $-0.47$ & $ 0.21$ &  0.17 &$-0.23$ & \nodata & $ 0.26$ & 0.00 &  0.07 &  0.15 \\
NYX014107       & Fe I  &  22 & $-0.68$ & $ 0.00$ &  0.14 &$-0.49$ & \nodata & $ 0.00$ & 0.00 &  0.04 &  0.13 \\
NYX014107       & Fe II &   7 & $-0.59$ & $ 0.09$ &  0.17 &$-0.40$ & \nodata & $ 0.09$ & 0.00 &  0.05 &  0.17 \\
NYX014107       & Ni I  &   6 & $-0.68$ & $-0.01$ &  0.14 &$-0.45$ & \nodata & $ 0.04$ & 0.00 &  0.05 &  0.13 \\
NYX014107       & Zn I  &   2 & $-0.35$ & $ 0.32$ &  0.13 &$-0.29$ & \nodata & $ 0.20$ & 0.01 &  0.03 &  0.12 \\
NYX014107       & Y II  &   4 & $-0.87$ & $-0.20$ &  0.19 &$-0.71$ & \nodata & $-0.22$ & 0.01 &  0.11 &  0.15 \\
NYX014107       & Ba II &   3 & $-0.69$ & $-0.02$ &  0.16 &$-0.66$ & \nodata & $-0.17$ & 0.00 &  0.00 &  0.16 \\
NYX014107       & La II &   1 & $-0.68$ & $-0.00$ &  0.16 &$-0.57$ & \nodata & $-0.08$ & 0.03 &  0.00 &  0.15 \\
NYX014725       & Na I  &   4 & $-0.05$ & $ 0.17$ &  0.14 &$-0.40$ & \nodata & $ 0.09$ & 0.00 &  0.10 &  0.10 \\
NYX014725       & Mg I  &   4 & $ 0.03$ & $ 0.25$ &  0.12 &$-0.10$ & \nodata & $ 0.39$ & 0.00 &  0.06 &  0.10 \\
NYX014725       & Si I  &   4 & $ 0.01$ & $ 0.23$ &  0.06 &$-0.14$ & \nodata & $ 0.35$ & 0.00 &  0.02 &  0.06 \\
NYX014725       & Ca I  &   7 & $-0.02$ & $ 0.20$ &  0.14 &$-0.28$ & \nodata & $ 0.21$ & 0.00 &  0.03 &  0.13 \\
NYX014725       & Ti I  &  11 & $-0.03$ & $ 0.19$ &  0.16 &$-0.23$ & \nodata & $ 0.26$ & 0.00 &  0.04 &  0.16 \\
NYX014725       & Fe I  &  22 & $-0.22$ & $ 0.00$ &  0.13 &$-0.49$ & \nodata & $ 0.00$ & 0.00 &  0.04 &  0.13 \\
NYX014725       & Fe II &   7 & $-0.13$ & $ 0.09$ &  0.19 &$-0.40$ & \nodata & $ 0.09$ & 0.00 &  0.05 &  0.18 \\
NYX014725       & Ni I  &   6 & $-0.19$ & $ 0.04$ &  0.13 &$-0.45$ & \nodata & $ 0.04$ & 0.00 &  0.05 &  0.12 \\
NYX014725       & Zn I  &   2 & $ 0.16$ & $ 0.38$ &  0.13 &$-0.29$ & \nodata & $ 0.20$ & 0.01 &  0.00 &  0.13 \\
NYX014725       & Y II  &   3 & $-0.33$ & $-0.11$ &  0.18 &$-0.71$ & \nodata & $-0.22$ & 0.01 &  0.09 &  0.16 \\
NYX014725       & Ba II &   3 & $-0.19$ & $ 0.04$ &  0.16 &$-0.66$ & \nodata & $-0.17$ & 0.00 &  0.06 &  0.15 \\
NYX014725       & La II &   1 & $-0.09$ & $ 0.13$ &  0.15 &$-0.57$ & \nodata & $-0.08$ & 0.02 &  0.00 &  0.15 \\
NYX022545       & Na I  &   4 & $-0.31$ & $ 0.01$ &  0.14 &$-0.40$ & \nodata & $ 0.09$ & 0.00 &  0.08 &  0.11 \\
NYX022545       & Mg I  &   4 & $-0.04$ & $ 0.28$ &  0.08 &$-0.10$ & \nodata & $ 0.39$ & 0.00 &  0.06 &  0.06 \\
NYX022545       & Si I  &   4 & $-0.05$ & $ 0.27$ &  0.12 &$-0.14$ & \nodata & $ 0.35$ & 0.00 &  0.06 &  0.11 \\
NYX022545       & Ca I  &   7 & $-0.14$ & $ 0.18$ &  0.18 &$-0.28$ & \nodata & $ 0.21$ & 0.00 &  0.09 &  0.16 \\
NYX022545       & Ti I  &  13 & $-0.01$ & $ 0.31$ &  0.19 &$-0.23$ & \nodata & $ 0.26$ & 0.00 &  0.04 &  0.19 \\
NYX022545       & Fe I  &  22 & $-0.32$ & $ 0.00$ &  0.13 &$-0.49$ & \nodata & $ 0.00$ & 0.00 &  0.05 &  0.12 \\
NYX022545       & Fe II &   6 & $-0.22$ & $ 0.10$ &  0.25 &$-0.40$ & \nodata & $ 0.09$ & 0.00 &  0.03 &  0.25 \\
NYX022545       & Ni I  &   6 & $-0.24$ & $ 0.08$ &  0.13 &$-0.45$ & \nodata & $ 0.04$ & 0.00 &  0.06 &  0.12 \\
NYX022545       & Zn I  &   1 & $-0.09$ & $ 0.23$ &  0.16 &$-0.29$ & \nodata & $ 0.20$ & 0.01 &  0.00 &  0.16 \\
NYX022545       & Y II  &   3 & $ 0.39$ & $ 0.71$ &  0.17 &$-0.71$ & \nodata & $-0.22$ & 0.00 &  0.05 &  0.16 \\
NYX022545       & Ba II &   3 & $ 0.58$ & $ 0.90$ &  0.18 &$-0.66$ & \nodata & $-0.17$ & 0.00 &  0.12 &  0.14 \\
NYX022545       & La II &   1 & $ 0.63$ & $ 0.95$ &  0.16 &$-0.57$ & \nodata & $-0.08$ & 0.02 &  0.00 &  0.16 \\
NYX035539       & Na I  &   4 & $-0.63$ & $ 0.04$ &  0.11 &$-0.40$ & \nodata & $ 0.09$ & 0.00 &  0.05 &  0.10 \\
NYX035539       & Mg I  &   4 & $-0.29$ & $ 0.38$ &  0.07 &$-0.10$ & \nodata & $ 0.39$ & 0.00 &  0.04 &  0.05 \\
NYX035539       & Si I  &   4 & $-0.34$ & $ 0.32$ &  0.11 &$-0.14$ & \nodata & $ 0.35$ & 0.00 &  0.04 &  0.10 \\
NYX035539       & Ca I  &   7 & $-0.37$ & $ 0.30$ &  0.15 &$-0.28$ & \nodata & $ 0.21$ & 0.00 &  0.02 &  0.15 \\
NYX035539       & Ti I  &  12 & $-0.33$ & $ 0.34$ &  0.18 &$-0.23$ & \nodata & $ 0.26$ & 0.00 &  0.04 &  0.17 \\
NYX035539       & Fe I  &  24 & $-0.67$ & $ 0.00$ &  0.11 &$-0.49$ & \nodata & $ 0.00$ & 0.00 &  0.04 &  0.10 \\
NYX035539       & Fe II &   6 & $-0.57$ & $ 0.09$ &  0.23 &$-0.40$ & \nodata & $ 0.09$ & 0.00 &  0.04 &  0.23 \\
NYX035539       & Ni I  &   6 & $-0.64$ & $ 0.02$ &  0.12 &$-0.45$ & \nodata & $ 0.04$ & 0.00 &  0.05 &  0.11 \\
NYX035539       & Zn I  &   2 & $-0.44$ & $ 0.22$ &  0.15 &$-0.29$ & \nodata & $ 0.20$ & 0.01 &  0.01 &  0.15 \\
NYX035539       & Y II  &   3 & $-0.65$ & $ 0.02$ &  0.16 &$-0.71$ & \nodata & $-0.22$ & 0.01 &  0.05 &  0.15 \\
NYX035539       & Ba II &   3 & $-0.63$ & $ 0.04$ &  0.17 &$-0.66$ & \nodata & $-0.17$ & 0.00 &  0.06 &  0.15 \\
NYX035539       & La II &   1 & $-0.52$ & $ 0.15$ &  0.14 &$-0.57$ & \nodata & $-0.08$ & 0.01 &  0.00 &  0.14 \\
NYX044831       & Na I  &   4 & $-0.90$ & $-0.04$ &  0.10 &$-0.40$ & \nodata & $ 0.09$ & 0.01 &  0.08 &  0.07 \\
NYX044831       & Mg I  &   3 & $-0.57$ & $ 0.30$ &  0.11 &$-0.10$ & \nodata & $ 0.39$ & 0.01 &  0.05 &  0.10 \\
NYX044831       & Si I  &   4 & $-0.53$ & $ 0.34$ &  0.06 &$-0.14$ & \nodata & $ 0.35$ & 0.00 &  0.03 &  0.05 \\
NYX044831       & Ca I  &   7 & $-0.50$ & $ 0.37$ &  0.21 &$-0.28$ & \nodata & $ 0.21$ & 0.01 &  0.18 &  0.11 \\
NYX044831       & Ti I  &   5 & $-0.67$ & $ 0.20$ &  0.16 &$-0.23$ & \nodata & $ 0.26$ & 0.01 &  0.11 &  0.12 \\
NYX044831       & Fe I  &  19 & $-0.86$ & $ 0.00$ &  0.13 &$-0.49$ & \nodata & $ 0.00$ & 0.00 &  0.06 &  0.11 \\
NYX044831       & Fe II &   6 & $-0.77$ & $ 0.09$ &  0.15 &$-0.40$ & \nodata & $ 0.09$ & 0.00 &  0.06 &  0.14 \\
NYX044831       & Ni I  &   5 & $-0.85$ & $ 0.01$ &  0.13 &$-0.45$ & \nodata & $ 0.04$ & 0.00 &  0.05 &  0.12 \\
NYX044831       & Zn I  &   2 & $-0.65$ & $ 0.21$ &  0.10 &$-0.29$ & \nodata & $ 0.20$ & 0.01 &  0.05 &  0.08 \\
NYX044831       & Y II  &   3 & $-1.20$ & $-0.33$ &  0.17 &$-0.71$ & \nodata & $-0.22$ & 0.01 &  0.12 &  0.13 \\
NYX044831       & Ba II &   3 & $-0.82$ & $ 0.05$ &  0.14 &$-0.66$ & \nodata & $-0.17$ & 0.01 &  0.01 &  0.14 \\
NYX044831       & La II &   1 & $-0.86$ & $-0.00$ &  0.14 &$-0.57$ & \nodata & $-0.08$ & 0.05 &  0.00 &  0.13 \\
NYX063721       & Na I  &   4 & $-0.40$ & $ 0.07$ &  0.11 &$-0.40$ & \nodata & $ 0.09$ & 0.00 &  0.06 &  0.10 \\
NYX063721       & Mg I  &   4 & $-0.15$ & $ 0.32$ &  0.12 &$-0.10$ & \nodata & $ 0.39$ & 0.00 &  0.05 &  0.11 \\
NYX063721       & Si I  &   4 & $-0.17$ & $ 0.29$ &  0.08 &$-0.14$ & \nodata & $ 0.35$ & 0.00 &  0.02 &  0.08 \\
NYX063721       & Ca I  &   7 & $-0.19$ & $ 0.27$ &  0.13 &$-0.28$ & \nodata & $ 0.21$ & 0.00 &  0.03 &  0.13 \\
NYX063721       & Ti I  &  12 & $-0.20$ & $ 0.27$ &  0.17 &$-0.23$ & \nodata & $ 0.26$ & 0.00 &  0.04 &  0.17 \\
NYX063721       & Fe I  &  24 & $-0.47$ & $ 0.00$ &  0.14 &$-0.49$ & \nodata & $ 0.00$ & 0.00 &  0.05 &  0.13 \\
NYX063721       & Fe II &   7 & $-0.38$ & $ 0.09$ &  0.20 &$-0.40$ & \nodata & $ 0.09$ & 0.00 &  0.06 &  0.19 \\
NYX063721       & Ni I  &   5 & $-0.47$ & $-0.00$ &  0.14 &$-0.45$ & \nodata & $ 0.04$ & 0.00 &  0.05 &  0.13 \\
NYX063721       & Zn I  &   2 & $-0.17$ & $ 0.30$ &  0.15 &$-0.29$ & \nodata & $ 0.20$ & 0.01 &  0.00 &  0.15 \\
NYX063721       & Y II  &   3 & $-0.59$ & $-0.12$ &  0.17 &$-0.71$ & \nodata & $-0.22$ & 0.01 &  0.02 &  0.17 \\
NYX063721       & Ba II &   3 & $-0.55$ & $-0.08$ &  0.17 &$-0.66$ & \nodata & $-0.17$ & 0.00 &  0.04 &  0.16 \\
NYX063721       & La II &   1 & $-0.50$ & $-0.03$ &  0.16 &$-0.57$ & \nodata & $-0.08$ & 0.03 &  0.00 &  0.16 \\
NYX064943       & Na I  &   4 & $-0.30$ & $ 0.06$ &  0.10 &$-0.40$ & \nodata & $ 0.09$ & 0.00 &  0.03 &  0.10 \\
NYX064943       & Mg I  &   4 & $-0.26$ & $ 0.10$ &  0.09 &$-0.10$ & \nodata & $ 0.39$ & 0.00 &  0.07 &  0.06 \\
NYX064943       & Si I  &   4 & $-0.19$ & $ 0.17$ &  0.10 &$-0.14$ & \nodata & $ 0.35$ & 0.00 &  0.02 &  0.09 \\
NYX064943       & Ca I  &   7 & $-0.22$ & $ 0.14$ &  0.15 &$-0.28$ & \nodata & $ 0.21$ & 0.00 &  0.05 &  0.14 \\
NYX064943       & Ti I  &  13 & $-0.31$ & $ 0.05$ &  0.18 &$-0.23$ & \nodata & $ 0.26$ & 0.00 &  0.05 &  0.18 \\
NYX064943       & Fe I  &  24 & $-0.36$ & $ 0.00$ &  0.12 &$-0.49$ & \nodata & $ 0.00$ & 0.00 &  0.04 &  0.12 \\
NYX064943       & Fe II &   7 & $-0.27$ & $ 0.09$ &  0.24 &$-0.40$ & \nodata & $ 0.09$ & 0.00 &  0.04 &  0.23 \\
NYX064943       & Ni I  &   6 & $-0.36$ & $-0.01$ &  0.13 &$-0.45$ & \nodata & $ 0.04$ & 0.00 &  0.04 &  0.12 \\
NYX064943       & Zn I  &   2 & $-0.25$ & $ 0.11$ &  0.17 &$-0.29$ & \nodata & $ 0.20$ & 0.01 &  0.07 &  0.16 \\
NYX064943       & Y II  &   3 & $-0.46$ & $-0.10$ &  0.17 &$-0.71$ & \nodata & $-0.22$ & 0.00 &  0.06 &  0.16 \\
NYX064943       & Ba II &   3 & $-0.15$ & $ 0.20$ &  0.18 &$-0.66$ & \nodata & $-0.17$ & 0.00 &  0.09 &  0.15 \\
NYX064943       & La II &   1 & $-0.21$ & $ 0.15$ &  0.15 &$-0.57$ & \nodata & $-0.08$ & 0.01 &  0.00 &  0.15 \\
NYX122147       & Na I  &   1 & $-2.09$ & $ 0.03$ &  0.14 &$-2.23$ &  0.08 & $-0.18$ & 0.02 &  0.00 &  0.14 \\
NYX122147       & Mg I  &   3 & $-1.54$ & $ 0.59$ &  0.27 &$-1.69$ &  0.03 & $ 0.36$ & 0.01 &  0.10 &  0.25 \\
NYX122147       & Si I  &   1 & $-1.80$ & $ 0.33$ &  0.11 &$-1.79$ &  0.11 & $ 0.26$ & 0.02 &  0.00 &  0.11 \\
NYX122147       & Ca I  &   5 & $-1.70$ & $ 0.43$ &  0.25 &$-1.84$ &  0.05 & $ 0.21$ & 0.01 &  0.10 &  0.23 \\
NYX122147       & Ti I  &  11 & $-2.03$ & $ 0.09$ &  0.35 &$-1.89$ &  0.10 & $ 0.16$ & 0.00 &  0.12 &  0.33 \\
NYX122147       & Fe I  &  13 & $-2.13$ & $ 0.00$ &  0.26 &$-2.05$ &  0.06 & $ 0.00$ & 0.00 &  0.06 &  0.25 \\
NYX122147       & Fe II &   7 & \nodata & \nodata &  0.18 &\nodata & \nodata & \nodata & 0.01 &  0.11 &  0.15 \\
NYX122147       & Ni I  &   6 & $-2.21$ & $-0.08$ &  0.26 &$-2.17$ &  0.08 & $-0.12$ & 0.01 &  0.05 &  0.25 \\
NYX122147       & Zn I  &   2 & \nodata & \nodata &  0.10 &\nodata & \nodata & \nodata & 0.01 &  0.02 &  0.10 \\
NYX122147       & Y II  &   3 & $-2.17$ & $-0.04$ &  0.16 &$-2.23$ &  0.18 & $-0.18$ & 0.01 &  0.06 &  0.15 \\
NYX122147       & Ba II &   3 & $-2.12$ & $ 0.00$ &  0.25 &$-2.22$ &  0.18 & $-0.17$ & 0.01 &  0.15 &  0.19 \\
NYX163705       & Na I  &   4 & $-0.50$ & $-0.03$ &  0.07 &$-0.37$ &  0.02 & $ 0.03$ & 0.00 &  0.04 &  0.06 \\
NYX163705       & Mg I  &   5 & $-0.16$ & $ 0.31$ &  0.10 &$-0.15$ &  0.02 & $ 0.25$ & 0.00 &  0.08 &  0.06 \\
NYX163705       & Si I  &   6 & $-0.33$ & $ 0.14$ &  0.06 &$-0.23$ &  0.03 & $ 0.17$ & 0.00 &  0.04 &  0.04 \\
NYX163705       & Ca I  &   6 & $-0.36$ & $ 0.11$ &  0.10 &$-0.29$ &  0.02 & $ 0.11$ & 0.00 &  0.05 &  0.09 \\
NYX163705       & Ti I  &  25 & $-0.14$ & $ 0.33$ &  0.12 &$-0.19$ &  0.01 & $ 0.21$ & 0.00 &  0.05 &  0.10 \\
NYX163705       & Fe I  &  20 & $-0.47$ & $ 0.00$ &  0.08 &$-0.40$ &  0.01 & $ 0.00$ & 0.00 &  0.03 &  0.08 \\
NYX163705       & Fe II &   5 & \nodata & \nodata &  0.11 &\nodata & \nodata & \nodata & 0.01 &  0.04 &  0.10 \\
NYX163705       & Ni I  &  12 & $-0.45$ & $ 0.03$ &  0.09 &$-0.40$ &  0.01 & $ 0.00$ & 0.00 &  0.04 &  0.08 \\
NYX163705       & Zn I  &   2 & $-0.34$ & $ 0.14$ &  0.08 &$-0.22$ &  0.02 & $ 0.18$ & 0.01 &  0.03 &  0.08 \\
NYX163705       & Y II  &   3 & $-0.35$ & $ 0.12$ &  0.11 &$-0.56$ &  0.03 & $-0.16$ & 0.01 &  0.04 &  0.10 \\
NYX163705       & Ba II &   3 & $-0.45$ & $ 0.02$ &  0.13 &$-0.47$ &  0.04 & $-0.07$ & 0.00 &  0.06 &  0.11 \\
NYX175752       & Na I  &   4 & $-0.44$ & $ 0.06$ &  0.11 &$-0.40$ & \nodata & $ 0.09$ & 0.00 &  0.05 &  0.10 \\
NYX175752       & Mg I  &   4 & $-0.09$ & $ 0.40$ &  0.07 &$-0.10$ & \nodata & $ 0.39$ & 0.00 &  0.02 &  0.06 \\
NYX175752       & Si I  &   4 & $-0.11$ & $ 0.38$ &  0.15 &$-0.14$ & \nodata & $ 0.35$ & 0.00 &  0.04 &  0.15 \\
NYX175752       & Ca I  &   7 & $-0.26$ & $ 0.23$ &  0.15 &$-0.28$ & \nodata & $ 0.21$ & 0.00 &  0.03 &  0.14 \\
NYX175752       & Ti I  &  12 & $-0.14$ & $ 0.35$ &  0.18 &$-0.23$ & \nodata & $ 0.26$ & 0.00 &  0.03 &  0.18 \\
NYX175752       & Fe I  &  22 & $-0.49$ & $ 0.00$ &  0.12 &$-0.49$ & \nodata & $ 0.00$ & 0.00 &  0.03 &  0.12 \\
NYX175752       & Fe II &   7 & $-0.40$ & $ 0.09$ &  0.29 &$-0.40$ & \nodata & $ 0.09$ & 0.00 &  0.03 &  0.28 \\
NYX175752       & Ni I  &   6 & $-0.45$ & $ 0.04$ &  0.14 &$-0.45$ & \nodata & $ 0.04$ & 0.00 &  0.03 &  0.13 \\
NYX175752       & Zn I  &   2 & $-0.36$ & $ 0.13$ &  0.19 &$-0.29$ & \nodata & $ 0.20$ & 0.01 &  0.01 &  0.19 \\
NYX175752       & Y II  &   3 & $-0.61$ & $-0.12$ &  0.18 &$-0.71$ & \nodata & $-0.22$ & 0.01 &  0.06 &  0.17 \\
NYX175752       & Ba II &   3 & $-0.61$ & $-0.12$ &  0.17 &$-0.66$ & \nodata & $-0.17$ & 0.00 &  0.01 &  0.17 \\
NYX175752       & La II &   1 & $-0.61$ & $-0.12$ &  0.13 &$-0.57$ & \nodata & $-0.08$ & 0.01 &  0.00 &  0.13 \\
NYX175906       & Na I  &   1 & $-1.72$ & $-0.01$ &  0.09 &$-2.23$ &  0.08 & $-0.18$ & 0.02 &  0.00 &  0.09 \\
NYX175906       & Mg I  &   3 & $-1.29$ & $ 0.42$ &  0.18 &$-1.69$ &  0.03 & $ 0.36$ & 0.00 &  0.05 &  0.18 \\
NYX175906       & Si I  &   1 & $-1.31$ & $ 0.40$ &  0.09 &$-1.79$ &  0.11 & $ 0.26$ & 0.01 &  0.00 &  0.09 \\
NYX175906       & Ca I  &   5 & $-1.34$ & $ 0.37$ &  0.18 &$-1.84$ &  0.05 & $ 0.21$ & 0.00 &  0.07 &  0.16 \\
NYX175906       & Ti I  &  11 & $-1.45$ & $ 0.26$ &  0.23 &$-1.89$ &  0.10 & $ 0.16$ & 0.00 &  0.09 &  0.21 \\
NYX175906       & Fe I  &  12 & $-1.71$ & $ 0.00$ &  0.18 &$-2.05$ &  0.06 & $ 0.00$ & 0.00 &  0.06 &  0.17 \\
NYX175906       & Fe II &   7 & \nodata & \nodata &  0.20 &\nodata & \nodata & \nodata & 0.00 &  0.13 &  0.15 \\
NYX175906       & Ni I  &   6 & $-1.73$ & $-0.02$ &  0.18 &$-2.17$ &  0.08 & $-0.12$ & 0.01 &  0.09 &  0.16 \\
NYX175906       & Zn I  &   2 & \nodata & \nodata &  0.13 &\nodata & \nodata & \nodata & 0.01 &  0.02 &  0.13 \\
NYX175906       & Y II  &   2 & $-1.40$ & $ 0.31$ &  0.19 &$-2.23$ &  0.18 & $-0.18$ & 0.01 &  0.04 &  0.18 \\
NYX175906       & Ba II &   3 & $-0.76$ & $ 0.95$ &  0.23 &$-2.22$ &  0.18 & $-0.17$ & 0.00 &  0.07 &  0.21 \\
NYX185250       & Na I  &   4 & $-0.75$ & $-0.10$ &  0.11 &$-0.40$ & \nodata & $ 0.09$ & 0.00 &  0.08 &  0.08 \\
NYX185250       & Mg I  &   4 & $-0.35$ & $ 0.31$ &  0.15 &$-0.10$ & \nodata & $ 0.39$ & 0.00 &  0.11 &  0.10 \\
NYX185250       & Si I  &   4 & $-0.39$ & $ 0.27$ &  0.06 &$-0.14$ & \nodata & $ 0.35$ & 0.00 &  0.03 &  0.05 \\
NYX185250       & Ca I  &   7 & $-0.44$ & $ 0.22$ &  0.15 &$-0.28$ & \nodata & $ 0.21$ & 0.00 &  0.09 &  0.12 \\
NYX185250       & Ti I  &   7 & $-0.49$ & $ 0.17$ &  0.16 &$-0.23$ & \nodata & $ 0.26$ & 0.00 &  0.08 &  0.13 \\
NYX185250       & Fe I  &  22 & $-0.66$ & $ 0.00$ &  0.14 &$-0.49$ & \nodata & $ 0.00$ & 0.00 &  0.06 &  0.12 \\
NYX185250       & Fe II &   7 & $-0.57$ & $ 0.09$ &  0.18 &$-0.40$ & \nodata & $ 0.09$ & 0.00 &  0.06 &  0.17 \\
NYX185250       & Ni I  &   6 & $-0.69$ & $-0.03$ &  0.13 &$-0.45$ & \nodata & $ 0.04$ & 0.00 &  0.06 &  0.12 \\
NYX185250       & Zn I  &   2 & $-0.41$ & $ 0.25$ &  0.13 &$-0.29$ & \nodata & $ 0.20$ & 0.01 &  0.02 &  0.13 \\
NYX185250       & Y II  &   2 & $-1.01$ & $-0.36$ &  0.15 &$-0.71$ & \nodata & $-0.22$ & 0.00 &  0.02 &  0.15 \\
NYX185250       & Ba II &   3 & $-0.63$ & $ 0.03$ &  0.16 &$-0.66$ & \nodata & $-0.17$ & 0.00 &  0.01 &  0.16 \\
NYX185250       & La II &   1 & $-0.61$ & $ 0.05$ &  0.14 &$-0.57$ & \nodata & $-0.08$ & 0.04 &  0.00 &  0.13 \\
NYX195253       & Na I  &   4 & $-0.50$ & $ 0.06$ &  0.06 &$-0.37$ &  0.02 & $ 0.03$ & 0.00 &  0.03 &  0.05 \\
NYX195253       & Mg I  &   5 & $-0.22$ & $ 0.34$ &  0.13 &$-0.15$ &  0.02 & $ 0.25$ & 0.00 &  0.11 &  0.06 \\
NYX195253       & Si I  &   6 & $-0.40$ & $ 0.15$ &  0.13 &$-0.23$ &  0.03 & $ 0.17$ & 0.00 &  0.12 &  0.04 \\
NYX195253       & Ca I  &   7 & $-0.33$ & $ 0.22$ &  0.09 &$-0.29$ &  0.02 & $ 0.11$ & 0.00 &  0.02 &  0.08 \\
NYX195253       & Ti I  &  24 & $-0.28$ & $ 0.27$ &  0.11 &$-0.19$ &  0.01 & $ 0.21$ & 0.00 &  0.04 &  0.11 \\
NYX195253       & Fe I  &  20 & $-0.56$ & $ 0.00$ &  0.09 &$-0.40$ &  0.01 & $ 0.00$ & 0.00 &  0.04 &  0.08 \\
NYX195253       & Fe II &   5 & \nodata & \nodata &  0.09 &\nodata & \nodata & \nodata & 0.00 &  0.02 &  0.09 \\
NYX195253       & Ni I  &  12 & $-0.54$ & $ 0.02$ &  0.09 &$-0.40$ &  0.01 & $ 0.00$ & 0.00 &  0.03 &  0.08 \\
NYX195253       & Zn I  &   2 & $-0.47$ & $ 0.09$ &  0.07 &$-0.22$ &  0.02 & $ 0.18$ & 0.01 &  0.02 &  0.07 \\
NYX195253       & Y II  &   3 & $-0.60$ & $-0.05$ &  0.11 &$-0.56$ &  0.03 & $-0.16$ & 0.01 &  0.04 &  0.11 \\
NYX195253       & Ba II &   3 & $-0.63$ & $-0.07$ &  0.10 &$-0.47$ &  0.04 & $-0.07$ & 0.00 &  0.03 &  0.10 \\
NYX201634       & Na I  &   4 & $-0.74$ & $-0.06$ &  0.13 &$-0.40$ & \nodata & $ 0.09$ & 0.00 &  0.10 &  0.08 \\
NYX201634       & Mg I  &   4 & $-0.42$ & $ 0.25$ &  0.09 &$-0.10$ & \nodata & $ 0.39$ & 0.00 &  0.03 &  0.09 \\
NYX201634       & Si I  &   4 & $-0.38$ & $ 0.30$ &  0.08 &$-0.14$ & \nodata & $ 0.35$ & 0.00 &  0.03 &  0.07 \\
NYX201634       & Ca I  &   7 & $-0.40$ & $ 0.27$ &  0.14 &$-0.28$ & \nodata & $ 0.21$ & 0.00 &  0.04 &  0.13 \\
NYX201634       & Ti I  &  11 & $-0.40$ & $ 0.28$ &  0.15 &$-0.23$ & \nodata & $ 0.26$ & 0.00 &  0.05 &  0.14 \\
NYX201634       & Fe I  &  22 & $-0.67$ & $ 0.00$ &  0.12 &$-0.49$ & \nodata & $ 0.00$ & 0.00 &  0.05 &  0.11 \\
NYX201634       & Fe II &   7 & $-0.58$ & $ 0.09$ &  0.19 &$-0.40$ & \nodata & $ 0.09$ & 0.00 &  0.04 &  0.18 \\
NYX201634       & Ni I  &   6 & $-0.66$ & $ 0.01$ &  0.12 &$-0.45$ & \nodata & $ 0.04$ & 0.00 &  0.05 &  0.11 \\
NYX201634       & Zn I  &   2 & $-0.38$ & $ 0.29$ &  0.13 &$-0.29$ & \nodata & $ 0.20$ & 0.01 &  0.02 &  0.13 \\
NYX201634       & Y II  &   3 & $-0.64$ & $ 0.03$ &  0.17 &$-0.71$ & \nodata & $-0.22$ & 0.01 &  0.07 &  0.15 \\
NYX201634       & Ba II &   3 & $-0.63$ & $ 0.04$ &  0.15 &$-0.66$ & \nodata & $-0.17$ & 0.00 &  0.04 &  0.14 \\
NYX201634       & La II &   1 & $-0.53$ & $ 0.14$ &  0.15 &$-0.57$ & \nodata & $-0.08$ & 0.03 &  0.00 &  0.15 \\
NYX201856       & Na I  &   4 & $-0.68$ & $ 0.02$ &  0.06 &$-0.37$ &  0.02 & $ 0.03$ & 0.00 &  0.04 &  0.04 \\
NYX201856       & Mg I  &   4 & $-0.34$ & $ 0.36$ &  0.06 &$-0.15$ &  0.02 & $ 0.25$ & 0.00 &  0.02 &  0.06 \\
NYX201856       & Si I  &   6 & $-0.55$ & $ 0.14$ &  0.12 &$-0.23$ &  0.03 & $ 0.17$ & 0.00 &  0.12 &  0.03 \\
NYX201856       & Ca I  &   7 & $-0.46$ & $ 0.24$ &  0.07 &$-0.29$ &  0.02 & $ 0.11$ & 0.00 &  0.02 &  0.07 \\
NYX201856       & Ti I  &  25 & $-0.37$ & $ 0.33$ &  0.09 &$-0.19$ &  0.01 & $ 0.21$ & 0.00 &  0.05 &  0.07 \\
NYX201856       & Fe I  &  20 & $-0.70$ & $ 0.00$ &  0.07 &$-0.40$ &  0.01 & $ 0.00$ & 0.00 &  0.04 &  0.06 \\
NYX201856       & Fe II &   5 & \nodata & \nodata &  0.11 &\nodata & \nodata & \nodata & 0.01 &  0.05 &  0.09 \\
NYX201856       & Ni I  &  12 & $-0.69$ & $ 0.01$ &  0.07 &$-0.40$ &  0.01 & $ 0.00$ & 0.00 &  0.04 &  0.06 \\
NYX201856       & Zn I  &   2 & $-0.53$ & $ 0.17$ &  0.08 &$-0.22$ &  0.02 & $ 0.18$ & 0.01 &  0.02 &  0.08 \\
NYX201856       & Y II  &   3 & $-0.66$ & $ 0.04$ &  0.10 &$-0.56$ &  0.03 & $-0.16$ & 0.01 &  0.05 &  0.09 \\
NYX201856       & Ba II &   3 & $-0.68$ & $ 0.02$ &  0.10 &$-0.47$ &  0.04 & $-0.07$ & 0.00 &  0.04 &  0.10 \\
NYX204828       & Na I  &   4 & $-0.73$ & $-0.02$ &  0.11 &$-0.40$ & \nodata & $ 0.09$ & 0.00 &  0.04 &  0.10 \\
NYX204828       & Mg I  &   4 & $-0.34$ & $ 0.37$ &  0.08 &$-0.10$ & \nodata & $ 0.39$ & 0.00 &  0.05 &  0.06 \\
NYX204828       & Si I  &   4 & $-0.37$ & $ 0.34$ &  0.11 &$-0.14$ & \nodata & $ 0.35$ & 0.00 &  0.05 &  0.09 \\
NYX204828       & Ca I  &   7 & $-0.41$ & $ 0.31$ &  0.15 &$-0.28$ & \nodata & $ 0.21$ & 0.00 &  0.04 &  0.14 \\
NYX204828       & Ti I  &  11 & $-0.41$ & $ 0.31$ &  0.18 &$-0.23$ & \nodata & $ 0.26$ & 0.00 &  0.05 &  0.17 \\
NYX204828       & Fe I  &  22 & $-0.71$ & $ 0.00$ &  0.11 &$-0.49$ & \nodata & $ 0.00$ & 0.00 &  0.03 &  0.11 \\
NYX204828       & Fe II &   7 & $-0.62$ & $ 0.09$ &  0.22 &$-0.40$ & \nodata & $ 0.09$ & 0.00 &  0.03 &  0.22 \\
NYX204828       & Ni I  &   6 & $-0.71$ & $ 0.01$ &  0.12 &$-0.45$ & \nodata & $ 0.04$ & 0.00 &  0.04 &  0.11 \\
NYX204828       & Zn I  &   2 & $-0.52$ & $ 0.20$ &  0.15 &$-0.29$ & \nodata & $ 0.20$ & 0.01 &  0.02 &  0.15 \\
NYX204828       & Y II  &   2 & $-0.69$ & $ 0.02$ &  0.16 &$-0.71$ & \nodata & $-0.22$ & 0.00 &  0.02 &  0.16 \\
NYX204828       & Ba II &   3 & $-0.66$ & $ 0.06$ &  0.16 &$-0.66$ & \nodata & $-0.17$ & 0.00 &  0.04 &  0.16 \\
NYX204828       & La II &   1 & $-0.61$ & $ 0.10$ &  0.14 &$-0.57$ & \nodata & $-0.08$ & 0.01 &  0.00 &  0.14 \\
NYX205642       & Na I  &   4 & $-0.53$ & $-0.07$ &  0.17 &$-0.40$ & \nodata & $ 0.09$ & 0.00 &  0.14 &  0.09 \\
NYX205642       & Mg I  &   4 & $-0.19$ & $ 0.28$ &  0.14 &$-0.10$ & \nodata & $ 0.39$ & 0.00 &  0.10 &  0.09 \\
NYX205642       & Si I  &   4 & $-0.24$ & $ 0.22$ &  0.09 &$-0.14$ & \nodata & $ 0.35$ & 0.00 &  0.06 &  0.07 \\
NYX205642       & Ca I  &   7 & $-0.29$ & $ 0.17$ &  0.15 &$-0.28$ & \nodata & $ 0.21$ & 0.00 &  0.06 &  0.14 \\
NYX205642       & Ti I  &  11 & $-0.19$ & $ 0.28$ &  0.17 &$-0.23$ & \nodata & $ 0.26$ & 0.00 &  0.09 &  0.15 \\
NYX205642       & Fe I  &  22 & $-0.47$ & $ 0.00$ &  0.13 &$-0.49$ & \nodata & $ 0.00$ & 0.00 &  0.07 &  0.11 \\
NYX205642       & Fe II &   7 & $-0.38$ & $ 0.09$ &  0.19 &$-0.40$ & \nodata & $ 0.09$ & 0.00 &  0.02 &  0.19 \\
NYX205642       & Ni I  &   6 & $-0.45$ & $ 0.02$ &  0.13 &$-0.45$ & \nodata & $ 0.04$ & 0.00 &  0.07 &  0.11 \\
NYX205642       & Zn I  &   2 & $-0.23$ & $ 0.24$ &  0.12 &$-0.29$ & \nodata & $ 0.20$ & 0.01 &  0.01 &  0.12 \\
NYX205642       & Y II  &   3 & $-0.63$ & $-0.16$ &  0.17 &$-0.71$ & \nodata & $-0.22$ & 0.01 &  0.07 &  0.16 \\
NYX205642       & Ba II &   3 & $-0.57$ & $-0.10$ &  0.15 &$-0.66$ & \nodata & $-0.17$ & 0.00 &  0.06 &  0.14 \\
NYX205642       & La II &   1 & $-0.34$ & $ 0.13$ &  0.16 &$-0.57$ & \nodata & $-0.08$ & 0.04 &  0.00 &  0.15 \\
NYX211145       & Na I  &   4 & $-0.61$ & $-0.03$ &  0.14 &$-0.40$ & \nodata & $ 0.09$ & 0.00 &  0.10 &  0.09 \\
NYX211145       & Mg I  &   4 & $-0.29$ & $ 0.29$ &  0.12 &$-0.10$ & \nodata & $ 0.39$ & 0.00 &  0.07 &  0.09 \\
NYX211145       & Si I  &   4 & $-0.31$ & $ 0.27$ &  0.09 &$-0.14$ & \nodata & $ 0.35$ & 0.00 &  0.05 &  0.08 \\
NYX211145       & Ca I  &   7 & $-0.34$ & $ 0.23$ &  0.15 &$-0.28$ & \nodata & $ 0.21$ & 0.00 &  0.05 &  0.14 \\
NYX211145       & Ti I  &  11 & $-0.25$ & $ 0.33$ &  0.17 &$-0.23$ & \nodata & $ 0.26$ & 0.00 &  0.06 &  0.16 \\
NYX211145       & Fe I  &  22 & $-0.58$ & $ 0.00$ &  0.13 &$-0.49$ & \nodata & $ 0.00$ & 0.00 &  0.06 &  0.11 \\
NYX211145       & Fe II &   7 & $-0.49$ & $ 0.09$ &  0.20 &$-0.40$ & \nodata & $ 0.09$ & 0.00 &  0.04 &  0.20 \\
NYX211145       & Ni I  &   6 & $-0.55$ & $ 0.03$ &  0.12 &$-0.45$ & \nodata & $ 0.04$ & 0.00 &  0.05 &  0.11 \\
NYX211145       & Zn I  &   2 & $-0.35$ & $ 0.23$ &  0.14 &$-0.29$ & \nodata & $ 0.20$ & 0.01 &  0.01 &  0.14 \\
NYX211145       & Y II  &   2 & $-0.52$ & $ 0.06$ &  0.18 &$-0.71$ & \nodata & $-0.22$ & 0.01 &  0.07 &  0.16 \\
NYX211145       & Ba II &   3 & $-0.64$ & $-0.06$ &  0.15 &$-0.66$ & \nodata & $-0.17$ & 0.00 &  0.04 &  0.15 \\
NYX211145       & La II &   1 & $-0.50$ & $ 0.08$ &  0.15 &$-0.57$ & \nodata & $-0.08$ & 0.03 &  0.00 &  0.14 \\
NYX213012       & Na I  &   1 & $-2.19$ & $-0.11$ &  0.11 &$-2.23$ &  0.08 & $-0.18$ & 0.02 &  0.00 &  0.11 \\
NYX213012       & Mg I  &   3 & $-1.63$ & $ 0.46$ &  0.21 &$-1.69$ &  0.03 & $ 0.36$ & 0.00 &  0.06 &  0.21 \\
NYX213012       & Si I  &   1 & $-1.66$ & $ 0.42$ &  0.10 &$-1.79$ &  0.11 & $ 0.26$ & 0.01 &  0.00 &  0.10 \\
NYX213012       & Ca I  &   5 & $-1.69$ & $ 0.39$ &  0.21 &$-1.84$ &  0.05 & $ 0.21$ & 0.00 &  0.09 &  0.20 \\
NYX213012       & Ti I  &  11 & $-1.94$ & $ 0.14$ &  0.28 &$-1.89$ &  0.10 & $ 0.16$ & 0.00 &  0.11 &  0.26 \\
NYX213012       & Fe I  &  13 & $-2.08$ & $ 0.00$ &  0.22 &$-2.05$ &  0.06 & $ 0.00$ & 0.00 &  0.06 &  0.21 \\
NYX213012       & Fe II &   7 & \nodata & \nodata &  0.15 &\nodata & \nodata & \nodata & 0.00 &  0.08 &  0.13 \\
NYX213012       & Ni I  &   6 & $-2.09$ & $-0.01$ &  0.22 &$-2.17$ &  0.08 & $-0.12$ & 0.00 &  0.10 &  0.20 \\
NYX213012       & Zn I  &   2 & \nodata & \nodata &  0.11 &\nodata & \nodata & \nodata & 0.01 &  0.03 &  0.10 \\
NYX213012       & Y II  &   2 & $-2.13$ & $-0.05$ &  0.15 &$-2.23$ &  0.18 & $-0.18$ & 0.01 &  0.00 &  0.15 \\
NYX213012       & Ba II &   3 & $-2.11$ & $-0.02$ &  0.32 &$-2.22$ &  0.18 & $-0.17$ & 0.01 &  0.26 &  0.18 \\
NYX214142       & Na I  &   4 & $-0.78$ & $-0.04$ &  0.09 &$-0.40$ & \nodata & $ 0.09$ & 0.00 &  0.07 &  0.06 \\
NYX214142       & Mg I  &   3 & $-0.46$ & $ 0.28$ &  0.11 &$-0.10$ & \nodata & $ 0.39$ & 0.01 &  0.06 &  0.09 \\
NYX214142       & Si I  &   4 & $-0.48$ & $ 0.26$ &  0.06 &$-0.14$ & \nodata & $ 0.35$ & 0.00 &  0.05 &  0.04 \\
NYX214142       & Ca I  &   7 & $-0.53$ & $ 0.21$ &  0.13 &$-0.28$ & \nodata & $ 0.21$ & 0.00 &  0.08 &  0.11 \\
NYX214142       & Ti I  &   8 & $-0.62$ & $ 0.12$ &  0.15 &$-0.23$ & \nodata & $ 0.26$ & 0.00 &  0.09 &  0.12 \\
NYX214142       & Fe I  &  22 & $-0.74$ & $ 0.00$ &  0.12 &$-0.49$ & \nodata & $ 0.00$ & 0.00 &  0.05 &  0.11 \\
NYX214142       & Fe II &   7 & $-0.65$ & $ 0.09$ &  0.16 &$-0.40$ & \nodata & $ 0.09$ & 0.00 &  0.06 &  0.15 \\
NYX214142       & Ni I  &   6 & $-0.76$ & $-0.02$ &  0.12 &$-0.45$ & \nodata & $ 0.04$ & 0.00 &  0.05 &  0.11 \\
NYX214142       & Zn I  &   2 & $-0.49$ & $ 0.25$ &  0.11 &$-0.29$ & \nodata & $ 0.20$ & 0.01 &  0.05 &  0.10 \\
NYX214142       & Y II  &   4 & $-1.08$ & $-0.34$ &  0.17 &$-0.71$ & \nodata & $-0.22$ & 0.00 &  0.10 &  0.14 \\
NYX214142       & Ba II &   3 & $-0.72$ & $ 0.02$ &  0.14 &$-0.66$ & \nodata & $-0.17$ & 0.00 &  0.02 &  0.14 \\
NYX214142       & La II &   1 & $-0.80$ & $-0.06$ &  0.15 &$-0.57$ & \nodata & $-0.08$ & 0.05 &  0.00 &  0.15 \\
NYX215612       & Na I  &   4 & $-0.48$ & $ 0.02$ &  0.06 &$-0.37$ &  0.02 & $ 0.03$ & 0.00 &  0.03 &  0.06 \\
NYX215612       & Mg I  &   4 & $-0.25$ & $ 0.25$ &  0.08 &$-0.15$ &  0.02 & $ 0.25$ & 0.00 &  0.03 &  0.07 \\
NYX215612       & Si I  &   6 & $-0.40$ & $ 0.11$ &  0.11 &$-0.23$ &  0.03 & $ 0.17$ & 0.00 &  0.11 &  0.03 \\
NYX215612       & Ca I  &   7 & $-0.40$ & $ 0.11$ &  0.09 &$-0.29$ &  0.02 & $ 0.11$ & 0.00 &  0.02 &  0.09 \\
NYX215612       & Ti I  &  24 & $-0.27$ & $ 0.24$ &  0.12 &$-0.19$ &  0.01 & $ 0.21$ & 0.00 &  0.05 &  0.11 \\
NYX215612       & Fe I  &  20 & $-0.51$ & $ 0.00$ &  0.10 &$-0.40$ &  0.01 & $ 0.00$ & 0.00 &  0.05 &  0.09 \\
NYX215612       & Fe II &   5 & \nodata & \nodata &  0.09 &\nodata & \nodata & \nodata & 0.00 &  0.03 &  0.08 \\
NYX215612       & Ni I  &  12 & $-0.52$ & $-0.01$ &  0.10 &$-0.40$ &  0.01 & $ 0.00$ & 0.00 &  0.05 &  0.08 \\
NYX215612       & Zn I  &   2 & $-0.45$ & $ 0.06$ &  0.06 &$-0.22$ &  0.02 & $ 0.18$ & 0.01 &  0.01 &  0.06 \\
NYX215612       & Y II  &   3 & $-0.55$ & $-0.04$ &  0.09 &$-0.56$ &  0.03 & $-0.16$ & 0.01 &  0.03 &  0.08 \\
NYX215612       & Ba II &   3 & $-0.53$ & $-0.02$ &  0.10 &$-0.47$ &  0.04 & $-0.07$ & 0.00 &  0.03 &  0.09 \\
NYX215744       & Na I  &   4 & $-0.27$ & $-0.07$ &  0.20 &$-0.40$ & \nodata & $ 0.09$ & 0.00 &  0.17 &  0.11 \\
NYX215744       & Mg I  &   4 & $ 0.06$ & $ 0.26$ &  0.12 &$-0.10$ & \nodata & $ 0.39$ & 0.00 &  0.08 &  0.09 \\
NYX215744       & Si I  &   4 & $ 0.04$ & $ 0.24$ &  0.09 &$-0.14$ & \nodata & $ 0.35$ & 0.00 &  0.03 &  0.08 \\
NYX215744       & Ca I  &   7 & $-0.07$ & $ 0.13$ &  0.16 &$-0.28$ & \nodata & $ 0.21$ & 0.00 &  0.06 &  0.15 \\
NYX215744       & Ti I  &  12 & $ 0.07$ & $ 0.27$ &  0.16 &$-0.23$ & \nodata & $ 0.26$ & 0.00 &  0.05 &  0.15 \\
NYX215744       & Fe I  &  22 & $-0.20$ & $ 0.00$ &  0.11 &$-0.49$ & \nodata & $ 0.00$ & 0.00 &  0.06 &  0.09 \\
NYX215744       & Fe II &   7 & $-0.11$ & $ 0.09$ &  0.21 &$-0.40$ & \nodata & $ 0.09$ & 0.00 &  0.03 &  0.21 \\
NYX215744       & Ni I  &   6 & $-0.12$ & $ 0.08$ &  0.11 &$-0.45$ & \nodata & $ 0.04$ & 0.00 &  0.05 &  0.10 \\
NYX215744       & Zn I  &   2 & $ 0.13$ & $ 0.33$ &  0.13 &$-0.29$ & \nodata & $ 0.20$ & 0.01 &  0.03 &  0.12 \\
NYX215744       & Y II  &   2 & $-0.45$ & $-0.25$ &  0.18 &$-0.71$ & \nodata & $-0.22$ & 0.01 &  0.09 &  0.15 \\
NYX215744       & Ba II &   3 & $-0.27$ & $-0.07$ &  0.15 &$-0.66$ & \nodata & $-0.17$ & 0.00 &  0.06 &  0.14 \\
NYX215744       & La II &   1 & $-0.20$ & $-0.00$ &  0.15 &$-0.57$ & \nodata & $-0.08$ & 0.04 &  0.00 &  0.14 \\
NYX223035       & Na I  &   4 & $-0.37$ & $ 0.01$ &  0.11 &$-0.40$ & \nodata & $ 0.09$ & 0.00 &  0.06 &  0.09 \\
NYX223035       & Mg I  &   4 & $-0.02$ & $ 0.36$ &  0.11 &$-0.10$ & \nodata & $ 0.39$ & 0.00 &  0.06 &  0.09 \\
NYX223035       & Si I  &   4 & $-0.06$ & $ 0.32$ &  0.07 &$-0.14$ & \nodata & $ 0.35$ & 0.00 &  0.03 &  0.06 \\
NYX223035       & Ca I  &   7 & $-0.17$ & $ 0.21$ &  0.13 &$-0.28$ & \nodata & $ 0.21$ & 0.00 &  0.03 &  0.13 \\
NYX223035       & Ti I  &  12 & $-0.15$ & $ 0.23$ &  0.15 &$-0.23$ & \nodata & $ 0.26$ & 0.00 &  0.05 &  0.14 \\
NYX223035       & Fe I  &  22 & $-0.38$ & $ 0.00$ &  0.12 &$-0.49$ & \nodata & $ 0.00$ & 0.00 &  0.03 &  0.11 \\
NYX223035       & Fe II &   7 & $-0.29$ & $ 0.09$ &  0.19 &$-0.40$ & \nodata & $ 0.09$ & 0.00 &  0.05 &  0.19 \\
NYX223035       & Ni I  &   6 & $-0.35$ & $ 0.03$ &  0.11 &$-0.45$ & \nodata & $ 0.04$ & 0.00 &  0.04 &  0.10 \\
NYX223035       & Zn I  &   2 & $ 0.02$ & $ 0.40$ &  0.13 &$-0.29$ & \nodata & $ 0.20$ & 0.01 &  0.01 &  0.13 \\
NYX223035       & Y II  &   2 & $-0.40$ & $-0.02$ &  0.16 &$-0.71$ & \nodata & $-0.22$ & 0.01 &  0.06 &  0.15 \\
NYX223035       & Ba II &   3 & $-0.40$ & $-0.02$ &  0.15 &$-0.66$ & \nodata & $-0.17$ & 0.00 &  0.03 &  0.15 \\
NYX223035       & La II &   1 & $-0.44$ & $-0.06$ &  0.14 &$-0.57$ & \nodata & $-0.08$ & 0.03 &  0.00 &  0.14 \\
NYX224245       & Na I  &   4 & $-0.20$ & $-0.07$ &  0.19 &$-0.40$ & \nodata & $ 0.09$ & 0.00 &  0.15 &  0.12 \\
NYX224245       & Mg I  &   4 & $ 0.07$ & $ 0.20$ &  0.11 &$-0.10$ & \nodata & $ 0.39$ & 0.00 &  0.05 &  0.10 \\
NYX224245       & Si I  &   4 & $ 0.10$ & $ 0.22$ &  0.09 &$-0.14$ & \nodata & $ 0.35$ & 0.00 &  0.03 &  0.09 \\
NYX224245       & Ca I  &   7 & $-0.01$ & $ 0.12$ &  0.18 &$-0.28$ & \nodata & $ 0.21$ & 0.00 &  0.07 &  0.17 \\
NYX224245       & Ti I  &  12 & $ 0.13$ & $ 0.25$ &  0.19 &$-0.23$ & \nodata & $ 0.26$ & 0.00 &  0.04 &  0.18 \\
NYX224245       & Fe I  &  22 & $-0.13$ & $ 0.00$ &  0.11 &$-0.49$ & \nodata & $ 0.00$ & 0.00 &  0.05 &  0.10 \\
NYX224245       & Fe II &   7 & $-0.03$ & $ 0.09$ &  0.23 &$-0.40$ & \nodata & $ 0.09$ & 0.01 &  0.04 &  0.23 \\
NYX224245       & Ni I  &   6 & $-0.05$ & $ 0.08$ &  0.11 &$-0.45$ & \nodata & $ 0.04$ & 0.00 &  0.04 &  0.10 \\
NYX224245       & Zn I  &   2 & $ 0.25$ & $ 0.38$ &  0.13 &$-0.29$ & \nodata & $ 0.20$ & 0.01 &  0.04 &  0.13 \\
NYX224245       & Y II  &   1 & $-0.25$ & $-0.12$ &  0.16 &$-0.71$ & \nodata & $-0.22$ & 0.01 &  0.00 &  0.16 \\
NYX224245       & Ba II &   3 & $-0.20$ & $-0.07$ &  0.16 &$-0.66$ & \nodata & $-0.17$ & 0.00 &  0.07 &  0.14 \\
NYX224245       & La II &   1 & $-0.05$ & $ 0.08$ &  0.15 &$-0.57$ & \nodata & $-0.08$ & 0.03 &  0.00 &  0.15 \\
NYX225510       & Na I  &   4 & $-0.59$ & $ 0.07$ &  0.08 &$-0.37$ &  0.02 & $ 0.03$ & 0.00 &  0.05 &  0.06 \\
NYX225510       & Mg I  &   4 & $-0.35$ & $ 0.31$ &  0.08 &$-0.15$ &  0.02 & $ 0.25$ & 0.00 &  0.02 &  0.08 \\
NYX225510       & Si I  &   6 & $-0.50$ & $ 0.16$ &  0.12 &$-0.23$ &  0.03 & $ 0.17$ & 0.00 &  0.11 &  0.05 \\
NYX225510       & Ca I  &   7 & $-0.45$ & $ 0.21$ &  0.09 &$-0.29$ &  0.02 & $ 0.11$ & 0.00 &  0.02 &  0.09 \\
NYX225510       & Ti I  &  24 & $-0.38$ & $ 0.28$ &  0.12 &$-0.19$ &  0.01 & $ 0.21$ & 0.00 &  0.03 &  0.11 \\
NYX225510       & Fe I  &  20 & $-0.66$ & $ 0.00$ &  0.10 &$-0.40$ &  0.01 & $ 0.00$ & 0.00 &  0.05 &  0.09 \\
NYX225510       & Fe II &   5 & \nodata & \nodata &  0.08 &\nodata & \nodata & \nodata & 0.00 &  0.04 &  0.07 \\
NYX225510       & Ni I  &  12 & $-0.65$ & $ 0.01$ &  0.09 &$-0.40$ &  0.01 & $ 0.00$ & 0.00 &  0.03 &  0.09 \\
NYX225510       & Zn I  &   2 & $-0.51$ & $ 0.15$ &  0.07 &$-0.22$ &  0.02 & $ 0.18$ & 0.00 &  0.01 &  0.07 \\
NYX225510       & Y II  &   3 & $-0.68$ & $-0.02$ &  0.09 &$-0.56$ &  0.03 & $-0.16$ & 0.00 &  0.04 &  0.08 \\
NYX225510       & Ba II &   3 & $-0.69$ & $-0.03$ &  0.09 &$-0.47$ &  0.04 & $-0.07$ & 0.00 &  0.03 &  0.09 \\
NYX225510       & La II & 1.0 & $-0.58$ & $ 0.08$ &  0.22 &$-0.35$ & \nodata & $ 0.05$ & 0.09 &  0.20 &  0.05 \\
NYX230605       & Na I  &   4 & $-0.33$ & $ 0.09$ &  0.10 &$-0.37$ &  0.02 & $ 0.03$ & 0.01 &  0.09 &  0.05 \\
NYX230605       & Mg I  &   3 & $-0.25$ & $ 0.17$ &  0.08 &$-0.15$ &  0.02 & $ 0.25$ & 0.01 &  0.03 &  0.07 \\
NYX230605       & Si I  &   6 & $-0.27$ & $ 0.15$ &  0.13 &$-0.23$ &  0.03 & $ 0.17$ & 0.01 &  0.12 &  0.04 \\
NYX230605       & Ca I  &   7 & $-0.16$ & $ 0.26$ &  0.16 &$-0.29$ &  0.02 & $ 0.11$ & 0.00 &  0.14 &  0.08 \\
NYX230605       & Ti I  &  15 & $-0.12$ & $ 0.30$ &  0.11 &$-0.19$ &  0.01 & $ 0.21$ & 0.00 &  0.07 &  0.09 \\
NYX230605       & Fe I  &  14 & $-0.42$ & $ 0.00$ &  0.09 &$-0.40$ &  0.01 & $ 0.00$ & 0.00 &  0.05 &  0.07 \\
NYX230605       & Fe II &   5 & \nodata & \nodata &  0.08 &\nodata & \nodata & \nodata & 0.00 &  0.04 &  0.06 \\
NYX230605       & Ni I  &   9 & $-0.39$ & $ 0.03$ &  0.10 &$-0.40$ &  0.01 & $ 0.00$ & 0.00 &  0.07 &  0.08 \\
NYX230605       & Zn I  &   2 & $-0.37$ & $ 0.05$ &  0.07 &$-0.22$ &  0.02 & $ 0.18$ & 0.01 &  0.02 &  0.07 \\
NYX230605       & Y II  &   3 & $-0.45$ & $-0.03$ &  0.09 &$-0.56$ &  0.03 & $-0.16$ & 0.01 &  0.05 &  0.08 \\
NYX230605       & Ba II &   3 & $-0.25$ & $ 0.17$ &  0.15 &$-0.47$ &  0.04 & $-0.07$ & 0.01 &  0.11 &  0.10 \\
NYX230903       & Na I  &   1 & $-1.41$ & $-0.06$ &  0.10 &$-2.23$ &  0.08 & $-0.18$ & 0.01 &  0.00 &  0.10 \\
NYX230903       & Mg I  &   3 & $-1.00$ & $ 0.35$ &  0.21 &$-1.69$ &  0.03 & $ 0.36$ & 0.00 &  0.04 &  0.21 \\
NYX230903       & Si I  &   2 & $-1.22$ & $ 0.13$ &  0.14 &$-1.79$ &  0.11 & $ 0.26$ & 0.01 &  0.11 &  0.08 \\
NYX230903       & Ca I  &   5 & $-1.08$ & $ 0.27$ &  0.20 &$-1.84$ &  0.05 & $ 0.21$ & 0.00 &  0.03 &  0.20 \\
NYX230903       & Ti I  &  11 & $-1.24$ & $ 0.11$ &  0.25 &$-1.89$ &  0.10 & $ 0.16$ & 0.00 &  0.09 &  0.23 \\
NYX230903       & Fe I  &  12 & $-1.35$ & $ 0.00$ &  0.19 &$-2.05$ &  0.06 & $ 0.00$ & 0.00 &  0.07 &  0.18 \\
NYX230903       & Fe II &   7 & \nodata & \nodata &  0.18 &\nodata & \nodata & \nodata & 0.00 &  0.05 &  0.17 \\
NYX230903       & Ni I  &   6 & $-1.46$ & $-0.11$ &  0.19 &$-2.17$ &  0.08 & $-0.12$ & 0.00 &  0.07 &  0.17 \\
NYX230903       & Zn I  &   2 & \nodata & \nodata &  0.13 &\nodata & \nodata & \nodata & 0.01 &  0.06 &  0.12 \\
NYX230903       & Y II  &   2 & $-1.23$ & $ 0.12$ &  0.18 &$-2.23$ &  0.18 & $-0.18$ & 0.01 &  0.03 &  0.18 \\
NYX230903       & Ba II &   3 & $-1.37$ & $-0.02$ &  0.21 &$-2.22$ &  0.18 & $-0.17$ & 0.00 &  0.12 &  0.17 \\
NYX232032       & Na I  &   4 & $-0.84$ & $-0.03$ &  0.12 &$-0.40$ & \nodata & $ 0.09$ & 0.00 &  0.09 &  0.09 \\
NYX232032       & Mg I  &   3 & $-0.55$ & $ 0.25$ &  0.12 &$-0.10$ & \nodata & $ 0.39$ & 0.00 &  0.06 &  0.11 \\
NYX232032       & Si I  &   4 & $-0.54$ & $ 0.26$ &  0.07 &$-0.14$ & \nodata & $ 0.35$ & 0.00 &  0.04 &  0.06 \\
NYX232032       & Ca I  &   7 & $-0.59$ & $ 0.22$ &  0.14 &$-0.28$ & \nodata & $ 0.21$ & 0.00 &  0.04 &  0.13 \\
NYX232032       & Ti I  &  11 & $-0.56$ & $ 0.24$ &  0.16 &$-0.23$ & \nodata & $ 0.26$ & 0.00 &  0.07 &  0.15 \\
NYX232032       & Fe I  &  22 & $-0.80$ & $ 0.00$ &  0.13 &$-0.49$ & \nodata & $ 0.00$ & 0.00 &  0.04 &  0.12 \\
NYX232032       & Fe II &   7 & $-0.71$ & $ 0.09$ &  0.19 &$-0.40$ & \nodata & $ 0.09$ & 0.00 &  0.07 &  0.18 \\
NYX232032       & Ni I  &   6 & $-0.76$ & $ 0.04$ &  0.13 &$-0.45$ & \nodata & $ 0.04$ & 0.00 &  0.06 &  0.12 \\
NYX232032       & Zn I  &   2 & $-0.49$ & $ 0.31$ &  0.13 &$-0.29$ & \nodata & $ 0.20$ & 0.01 &  0.05 &  0.12 \\
NYX232032       & Y II  &   4 & $-0.94$ & $-0.14$ &  0.17 &$-0.71$ & \nodata & $-0.22$ & 0.01 &  0.09 &  0.15 \\
NYX232032       & Ba II &   3 & $-0.80$ & $ 0.00$ &  0.16 &$-0.66$ & \nodata & $-0.17$ & 0.00 &  0.06 &  0.15 \\
NYX232032       & La II &   1 & $-0.67$ & $ 0.13$ &  0.15 &$-0.57$ & \nodata & $-0.08$ & 0.05 &  0.00 &  0.14 \\
NYX234631       & Na I  &   4 & $-0.75$ & $ 0.07$ &  0.08 &$-0.37$ &  0.02 & $ 0.03$ & 0.00 &  0.06 &  0.06 \\
NYX234631       & Mg I  &   4 & $-0.47$ & $ 0.35$ &  0.10 &$-0.15$ &  0.02 & $ 0.25$ & 0.00 &  0.05 &  0.08 \\
NYX234631       & Si I  &   6 & $-0.63$ & $ 0.19$ &  0.14 &$-0.23$ &  0.03 & $ 0.17$ & 0.00 &  0.13 &  0.04 \\
NYX234631       & Ca I  &   7 & $-0.53$ & $ 0.30$ &  0.11 &$-0.29$ &  0.02 & $ 0.11$ & 0.00 &  0.05 &  0.10 \\
NYX234631       & Ti I  &  22 & $-0.57$ & $ 0.26$ &  0.14 &$-0.19$ &  0.01 & $ 0.21$ & 0.00 &  0.07 &  0.12 \\
NYX234631       & Fe I  &  18 & $-0.82$ & $ 0.00$ &  0.13 &$-0.40$ &  0.01 & $ 0.00$ & 0.00 &  0.09 &  0.09 \\
NYX234631       & Fe II &   5 & \nodata & \nodata &  0.10 &\nodata & \nodata & \nodata & 0.01 &  0.04 &  0.09 \\
NYX234631       & Ni I  &  12 & $-0.85$ & $-0.03$ &  0.13 &$-0.40$ &  0.01 & $ 0.00$ & 0.00 &  0.09 &  0.09 \\
NYX234631       & Zn I  &   2 & $-0.64$ & $ 0.18$ &  0.08 &$-0.22$ &  0.02 & $ 0.18$ & 0.01 &  0.03 &  0.07 \\
NYX234631       & Y II  &   3 & $-0.85$ & $-0.03$ &  0.11 &$-0.56$ &  0.03 & $-0.16$ & 0.01 &  0.06 &  0.10 \\
NYX234631       & Ba II &   3 & $-0.73$ & $ 0.09$ &  0.13 &$-0.47$ &  0.04 & $-0.07$ & 0.00 &  0.04 &  0.12 \\
\enddata
\tablecomments{One star from this table is shown for form. Column details are provided in the text. The full version is available online.}
\end{deluxetable*}

